$\mathcal{H}$-Killing Spinors and Spinorial Duality for Homogeneous 3-$(\alpha,\delta)$-Sasaki Manifolds

We show that $3$-$(\alpha,\delta)$-Sasaki manifolds admit solutions of a certain new spinorial field equation (the $\mathcal{H}$-Killing equation) generalizing the well-known Killing spinors on $3$-Sasakian manifolds. These $\mathcal{H}$-Killing spinors have more desirable geometric properties than the spinors obtained by simply deforming a $3$-Sasakian metric; in particular we obtain a one-to-one correspondence between $\mathcal{H}$-Killing spinors on dual pairs of homogeneous $3$-$(\alpha,\delta)$-Sasaki spaces. Finally, we show that $\mathcal{H}$-Killing spinors generalize certain special spinors in dimension $7$ previously constructed by Agricola-Friedrich and Agricola-Dileo using $\text{G}_2$-geometry.

==> main_body_canonically_parallel.tex <==
\section{Deformations of $\nabla$-Parallel Spinors}\label{section:canonically_parallel}

In this section we study solutions of the equation $\nabla \psi =0$ on a $\tad$ manifold, and describe how they change under $\mathcal{H}$-homothetic deformations. It is known from \cite[Cor.\@ 4.1.1]{3str} that the $\nabla$-holonomy algebra satisfies
\[
\mathfrak{hol}(\nabla) \subseteq (\mathfrak{sp}(n-1)\oplus \mathfrak{sp}(1)) \oplus \mathfrak{so}(3) \subset \mathfrak{so}(4n-4) \oplus \mathfrak{so}(3), 
\]
so if there is a $\nabla$-parallel spinor then this containment must be proper (since the lift of the standard action of $\mathfrak{so}(3)$ does not annihilate any element of the spinor module, see e.g.\@ \cite{Wang,AHLspheres}). An important example of this occurs for \emph{parallel} $\tad$ manifolds (i.e. those with $\beta:= 2(\delta-2\alpha)=0$), in which case it is known from \cite[Cor.\@ 4.1.2]{3str} that $\mathfrak{hol}(\nabla)\subseteq \mathfrak{sp}(n-1)$\todo{proper containment?} (this reduction occurs as a result of the identities in Proposition \ref{prelims:canonical_connection}, which imply that $\nabla\xi_i = \nabla \varphi_i =0$ in the parallel case). It is known that the spin lift of $\mathfrak{sp}(n-1) \subset \mathfrak{so}(4n-4)\oplus \mathfrak{so}(3)$ annihilates $2n$ vectors in the spin representation (see \cite[\S4]{AHLspheres}), and we obtain the following result:
\todo{make sure there isn't too much text overlap with the 7-dim section}

\begin{theorem}
	A parallel $\tad$ manifold admits at least $2n$ solutions of the equation $\nabla \psi = 0$. 
\end{theorem}
Solutions of $\nabla \psi =0$ arising in the parallel case are, a priori, unstable, in the sense that perturbing $\alpha,\delta$ can cause $\beta$ to become non-zero, increasing the size of $\mathfrak{hol}(\nabla)$. Philosophically, $\nabla$-parallel spinors should therefore occur as an isolated special case in a family of differential equations depending on $\alpha,\delta$. Using similar arguments as in the previous section, we describe in the following theorem the family of such equations obtained starting from a parallel $\tad$ structure and applying $\mathcal{H}$-homothetic deformations. 

Starting with a parallel $3$-$(\alpha_0,\delta_0)$-Sasaki structure ($\delta_0=2\alpha_0$), one checks that the parameters in Definition \ref{H_deformation_definition} needed to obtain a $\tad$ structure are
\[
a= \frac{2\alpha_0^2}{\alpha\delta}, \qquad b = \frac{2\alpha_0^2(2\alpha-\delta)}{\alpha\delta^2} ,\qquad c = \frac{2\alpha_0}{\delta}.
\]


\begin{theorem}
	A
\end{theorem}
\begin{proof}
	Recalling the the difference tensor $\tau$ from Lemma \ref{difference_tensor_lemma}, 
\end{proof}








